Eliminating the Barriers: Demystifying Wi-Fi Baseband Design and Introducing the PicoScenes Wi-Fi Sensing Platform

The research on Wi-Fi sensing has been thriving over the past decade but the process has not been smooth. Three barriers always hamper the research: unknown baseband design and its influence, inadequate hardware, and the lack of versatile and flexible measurement software. This paper tries to eliminate these barriers through the following work. First, we present an in-depth study of the baseband design of the Qualcomm Atheros AR9300 (QCA9300) NIC. We identify a missing item of the existing CSI model, namely, the CSI distortion, and identify the baseband filter as its origin. We also propose a distortion removal method. Second, we reintroduce both the QCA9300 and software-defined radio (SDR) as powerful hardware for research. For the QCA9300, we unlock the arbitrary tuning of both the carrier frequency and bandwidth. For SDR, we develop a high?performance software implementation of the 802.11a/g/n/ac/ax baseband, allowing users to fully control the baseband and access the complete physical-layer information. Third, we release the PicoScenes software, which supports concurrent CSI measure?ment from multiple QCA9300, Intel Wireless Link (IWL5300) and SDR hardware. PicoScenes features rich low-level controls, packet injection and software baseband implementation. It also allows users to develop their own measurement plugins. Finally, we report state-of-the-art results in the extensive evaluations of the PicoScenes system, such as the >2 GHz available spectrum on the QCA9300, concurrent CSI measurement, and up to 40 kHz and 1 kHz CSI measurement rates achieved by the QCA9300 and SDR. PicoScenes is available at https://ps.zpj.io.

==> acknowledgements.tex <==
%!TEX root = main.tex
This work is supported by Natural Science Foundation of China (NSFC) No. 61802291 and No.61502374, National Postdoctoral Program for Innovative Talent No. BX20180235, and Fundamental Research Funds for the Central Universities No. JB190304.

==> slope.tex <==
%!TEX root = main.tex

% 在wifi sensing中，phase slope极为重要，它是 propagation path distance的一个直接指标。而距离测量是wifi sensing一个非常重要的功能。

% 在前人的指标中，大家已经明确地指出phase中包含的误差成分。

% 我们对此做了一份实现，如图所示，两台时钟同步的USRP有线连接。 由于时钟同步，按理说两台机器最后测量到的CSI phase应该是稳定不变的，但是如图所示，CSI phase 仍然呈现随机特性。

% 经过深入研究，我们确认了一种由于multi-rate design导致的phase slope randomness，在multi-rate design条件下，即使两个机器都完全同步的，也可以产生phase slope randomness. 其原因如下图所示。

% 虽然Tx和Rx的timing完全同步，但是在higher rate -> lower rate resampling的时候，resample的时机却存在随机性。这种随机性就导致了。

==> tuning.tex <==
%!TEX root = main.tex

Measuring the exact CFO and SFO and analyzing them are substantial for COTS hardware based Wi-Fi sensing.
However, no previous work gives an exact measurement.
The large part of the reason is that the COTS NICs does not release the baseband signals for the OFDM symbols following HT-LTF, the absolute values of CFO and SFO cannot be measured by COTS NICs themselves.

In the following text, we first present the CFO and SFO measurement using PicoScenes on SDR, then we show the measurement results and analysis.


% CFO and SFO 是COTS hardware based Wi-Fi sensing最大的误差源之一，甚至对于专门的雷达系统也是一样。
% 然而，由于COTS网卡披露的信息极为有限，仅依靠现有的CSI信息，无法直接测量。
%测量并理解COTS网卡真实的CFO和SFO及其变化，对于Wi-Fi感知极为重要。在这一章，我们在PicoScenes平台的基础上，构建了SFO和CFO的精确测量。

% 在下面的文字，我们先介绍如何精确测量CFO和SFO，然后呈现测量的结果与分析

\begin{figure}[t]
    \centering 
    \includegraphics[width=0.9\columnwidth]{USRPTestbed_annotated.jpg}
    \caption{Testbed setup for CFO and SFO measurement. The signal transmitted by QCA9300 or IWL5300 (Tx) is 2-way split and fed into two USRP N210 equipped with UBX-40 daughterboard (Rx). OctoClock-G, with GPS signal locked, provides $<$1ppb level synchronized clocking for both USRP N210. The baseband signal received from both N210 is live decoded and measured by PicoScenes.}
    \label{fig:USRPTestBed}
\end{figure}

The evaluation setup is shown in Figure~\ref{fig:USRPTestBed}.

\subsection{Per Packet CFO and SFO measurement}




During the normal Wi-Fi frame decoding, CFO is estimated by the L-STF field, and SFO is not directly estimated but partially compensated by the pilot subcarriers.

Only the LTF fields 
Down into the signal level, Wi-Fi frame consists of preamble and data parts and the latter consist of multiple data symbols.
Normally, each packet has only one CSI and the data symbols are first equalized by the CSI and then decoded.

After decoding the frame, we can regenerate the data symbols with the same data and modulation scheme.

We regenerated data symbols with the decoded data and the same modulation scheme (MCS, coding type and scrambler initial seed).
Using the same CSI 
$H_{i}^{d} = Y_{i}^{d} / X_{i}^{d}$

Let $\Delta\mathbf{\theta}_{i}^{d} = \angle (H_{i+1}^{d} / H_{i}^{d})$ denote the phase difference between two adjacent data CSI vectors. 

The successively received data symbols are closely spaced in merely 3.6 or 4$\mu$s. In such short time, CFO and SFO are the only factors the makes the CSI different
$\Delta\mathbf{\theta}_{i}^{d} = 2\pi\Delta cf_{cfo} t_{SYM} + 2\pi k$
In this way, we literally transform the data symbols into a train of successively measured CSI. 
According to 802.11 standard, the duration of OFDM symbols is 3.6/4$\mu$s for short or long guard interval (GI).
The CSI measurements obtained from data symbols is 4$\mu$s evenly spaced.

\begin{equation}
    \arg \mathbf{H}_{i + 1}^{data} / \mathbf{H}_{i}^{data} = p[]
\end{equation}






Conventional Wi-Fi Rx end decode the 
